On the arithmetic Hilbert-Samuel theorem : a proof by deformation

We give a new proof the arithmetic Hilbert-Samuel theorem by using classical reductions in the theory of coherent sheaves, a direct proof in the case of the projective space and the conservation of some numerical invariants, called arithmetic Hilbert invariants, through the deformation to the projective completion of the cone. This construction lies at the intersection of deformation theory and Arakelov geometry. It provides a deformation of a Hermitian line bundle over the deformation to the normal cone.

==> 4-Deformation/hilbertsamuelarithmetique.tex <==
\subsection{Proof of the arithmetic Hilbert-Samuel theorem}


{\color{red} Les définitions sont déjà données.}


Différentes réductions possibles:\\

1) restriction pour immersion fermée\\
2) Dévissage \\

3) i) De $X$ à $X_{red}$\\
ii) De $F$ à $\mcO_X$ (Syzygy)\\
iii) De $X$ aux sous-variétés intègres.\\

Theorem: \\

Preuve:\\
